GitNet: Geometric Prior-based Transformation for Birds-Eye-View Segmentation

Birds-eye-view (BEV) semantic segmentation is critical for autonomous driving for its powerful spatial representation ability. It is challenging to estimate the BEV semantic maps from monocular images due to the spatial gap, since it is implicitly required to realize both the perspective-to-BEV transformation and segmentation. We present a novel two-stage Geometry Prior-based Transformation framework named GitNet, consisting of (i) the geometry-guided pre-alignment and (ii) ray-based transformer. In the first stage, we decouple the BEV segmentation into the perspective image segmentation and geometric prior-based mapping, with explicit supervision by projecting the BEV semantic labels onto the image plane to learn visibility-aware features and learnable geometry to translate into BEV space. Second, the pre-aligned coarse BEV features are further deformed by ray-based transformers to take visibility knowledge into account. GitNet achieves the leading performance on the challenging nuScenes and Argoverse Datasets.

==> experiment.tex <==
\section{Experiments}
\label{sec:experiments}


\subsection{Experimental Setup}

\noindent
\textbf{Datasets.} We conduct extensive experiments on two large-scale indoor datasets, ScanNet v2~\cite{dai2017scannet} and S3DIS~\cite{armeni20163d}. ScanNet v2 consists of 1,613 real-world 3D scenes with point-level semantic and instance annotations. The whole dataset is split into training, validation, and testing sets, each with 1201, 312, and 100 scans, respectively. It has 20 object categories, among which 18 (except the wall and floor) are commonly used for instance segmentation evaluation. S3DIS has 272 scanned 3D layouts across six large areas, including 13 different object categories. We follow the common split in previous work~\cite{jiang2020pointgroup,hou2021exploring} to adopt Area 5 as the validation set and the other five areas as the training set. 

\vspace*{2mm}
\noindent
\textbf{SSL Training Set Partition.} On ScanNet v2, we directly adopt the setting of ScanNet data-efficient benchmark~\cite{hou2021exploring}
% - {\em limited reconstructions} 
and split the training set into the labeled and unlabeled sets, with \{1\%, 5\%, 10\%, 20\%\} as the labeled data, respectively. Further, we follow these four labeling ratios to split S3DIS training set by randomly sampling the 3D scenes.

%\textbf{SSL Training Set Partition.} On ScanNet V2, we directly adopt the setting of ScanNet data-efficient benchmark - {\em limited reconstructions} and split the training set into labeled and unlabeled sets with \{1\%, 5\%, 10\%, 20\%\} of labeled data, respectively. For S3DIS, the training set is also split with these four labeled ratios by random sampling 3D scenes. 
% \ruihang{We further provide experimental results trained on more data, \ie, \{30\%, 40\%, 50\%\} training set, in supplementary materials to demonstrate the generalization capability of our method. Not determined....}

% You may read this book in the future: "Bugs in Writing"
\vspace*{2mm}
\noindent
\textbf{Implementation Details.} On both datasets, we train the 3D feature extraction network $\Phi$ and re-correction module $\Psi$ by the SGD optimizer, with a learning rate of 0.1 and 0.005, respectively. The learning rate is scheduled with the polynomial decay of power 0.9. In each round, our model is trained on four NVIDIA 2080Ti GPUs for 10k steps with a batch size of eight,~\ie, four labeled scenes and four unlabeled scenes. We adopt standard point cloud data augmentation strategies in~\cite{qi2019deep} to process 3D scenes before feeding them to $\Phi$. The bounding box scaling ratios for geometric mutation augmentations when training $\Psi$ are
within [0.7, 1.3]. For all experiments, we adopt the same Sparse U-Net~\cite{xie2020pointcontrast,hou2021exploring} as the backbone of $\Phi$ and a much smaller decoder,~\ie, with fewer layers and stages, as the backbone of $\Psi$. The Sparse ConvNet of the backbone is implemented by MinkowskiEngine~\cite{choy20194d}, with a voxel size of 2.0 cm. The self-training converges in three or four rounds.

\begin{figure*}
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
		\includegraphics[width=1\linewidth]{latex/figures/visualization_scannet.pdf}
	\end{center}
\vspace*{-6mm}
\caption{Comparisons of visualization results with CSC (trained with only 5\% labeled scenes). Distinct instances have different colors.
}
\label{fig:visualization_scannet}
\vspace*{-0.3cm}
\end{figure*}

\begin{table}[]
\centering
\setlength{\tabcolsep}{9.5pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|l|ccc}
\specialrule{0.3pt}{0.1pt}{0pt}
\hline
 L.R. & Method & mAP & AP$_{50}$ & AP$_{25}$ \\
 \hline
 & \ourMethod{} & 32.8 & 52.9  & 66.8 \\
\multirow{-2}{*}{20\%} & \ourMethod{}+CSC~\cite{hou2021exploring} & 34.1 & 53.7 & 67.8 \\
\hline
& Our Baseline Oracle & 36.8 & 57.2 & 71.8 \\
% & SGPN~\cite{wang2018sgpn} & - & 11.3 & 22.2 \\
& 3D-SIS~\cite{hou20193d} & - & 18.7 & 35.7 \\
& GSPN~\cite{yi2019gspn} & 19.3 & 37.8 & 53.4 \\
& MTML~\cite{lahoud20193d} & 20.3 & 40.2 & 55.4 \\
& PointGroup~\cite{jiang2020pointgroup} & 34.8 & 56.9 & 71.3 \\
& 3D-MPA~\cite{engelmann20203d} & 35.3 & 59.1 & 72.4 \\
\multirow{-8}{*}{100\%} & DyCo3D~\cite{he2021dyco3d} & 35.4 & 57.6 & - \\
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Comparisons with approaches that are supervised by 100\% labels on ScanNet validation set. L.R. means the label ratio.}
\label{tab:comparison_oracle}
\vspace*{-0.2cm}
\end{table}

\subsection{Main Results}


We evaluate our \ourMethod{} and other recent methods on ScanNet v2 and S3DIS.
Table~\ref{tab:main_result} depicts quantitative results on their validation sets, with 1\%, 5\%, 10\% and 20\% labeled data for supervision.
Table~\ref{tab:scannettest} presents online comparison results on the test set of ScanNet v2 data-efficient benchmark\footnote{http://kaldir.vc.in.tum.de/scannet\_benchmark/data\_efficient/}.
The compared methods include (i) Baseline: %use only the labeled data for supervision only; 
adopt the baseline method in Sec.~\ref{sec:preliminary} on the labeled portion of the data;
(ii) PointContrast~\cite{xie2020pointcontrast}; (iii) CSC~\cite{hou2021exploring}; (iv) \ourMethod{}; and (v) \ourMethod{} with CSC-pretrained model as initialization.


As shown in Table~\ref{tab:main_result}, \ourMethod{} significantly improves the performance over the baselines by leveraging quantities of unlabeled data for model training. In contrast to the two SOTA approaches (ii) (iii) that leverage the unsupervised pre-training, \ourMethod{} can generate high-quality pseudo labels as explicit supervisions and surpasses them consistently on all metrics. A noteworthy finding is that, TWIST with the CSC-pre-trained weights  
as initialization in the first round (v) can further boost the performance as shown in the gray rows of Tables~\ref{tab:main_result} and~\ref{tab:scannettest}, revealing their complementary strengths to this task. Specifically, their cooperative performance even doubles the mAP on ScanNet validation set with 1\% labels and achieves 34.1\% mAP, given only 20\% labels. The latter is only 2.7\% lower than the fully-supervised baseline oracle and can be comparable to several recent competitive approaches trained with 100\% labels, as shown in Table~\ref{tab:comparison_oracle}.


%\lzz{As shown in Table~\ref{tab:main_result}}, \ourMethod~significantly improves the performance compared with the baselines by leveraging quantities of unlabeled data for model training. Compared to two SOTA approaches (2) (3) that tackle this problem through unsupervised pre-training, our method generates high-quality pseudo labels as explicit supervisions and outperforms them consistently on all metrics. A noteworthy finding is that, initializing model parameters of TWIST from CSC pre-trained weights to start step \textbf{(i)} in self-training can further lift the performance, indicating their orthogonal benefit to the task. As observed in gray rows of Table~\ref{tab:main_result} and Table~\ref{tab:scannettest}, their cooperation performance even doubles the mAP on ScanNet validation set with scarce labels (1\%), and achieves 34.1\% mAP given 20\% labels. The latter is only 2.7\% lower than the fully-supervised baseline oracle and can surpass several competitive approaches trained with 100\% labels, as shown in Table~\ref{tab:comparison_oracle}.

Fig.~\ref{fig:visualization_scannet} shows the visual comparisons between TWIST and CSC on the ScanNet v2 validation set. With only 5\% labeled data for training, TWIST can generate clean instance predictions and shows a high capability of separating spatially-close objects, such as similar adjacent chairs. 
% More quantitative results are exhibited in supplementary materials. 


\subsection{Ablation Study}
\label{subsec:ablation}
We also conduct ablation studies to evaluate the key designs in \ourMethod{}.
%For ablation study,
Unless otherwise specified, we evaluate on the ScanNet v2 validation set with 5\% training data labeled.


\vspace*{2mm}
\noindent
\textbf{Effects of different components in \ourMethod{}}
To analyze the effects of the core components, we try different combinations and summarize the ablation results in Table~\ref{tab:abla_component}.
We first set the baseline as Group I. Based on it, the improvements are mainly derived from the following three aspects:
\begin{itemize}
\vspace{-2mm}
    \item \textbf{Pseudo labels.} Groups II and III generate pseudo semantic labels and pseudo offset vectors using the naive thresholding strategy discussed in Sec.~\ref{subsec:overview}, improving mAP by +2.7\% and +1.5\%, respectively. Their joint effect (Group IV) brings further gain (+0.4\% mAP).
    \vspace{-2mm}
    \item \textbf{Proposal-based pseudo-label update.} Group V exploits component \textbf{C} of \ourMethod{} (Fig.~\ref{fig:overview}) to generate proposal-level pseudo labels %pseudo labels in a proposal level, 
    and preserve pseudo-label consistency inside an instance proposal. Compared to the naive strategy (Group IV) for pseudo-labeling, the strategy enhances the performance by (+3.5\% mAP).
    \vspace{-2mm}
    \item \textbf{Re-correction module.} %The re-correction module provides an object-level denoise in two aspects. 
    This module contributes to the object-level pseudo-label denoising in two aspects.
    For instance proposals with instance certainty scores $\hat{v}_j$ lower than the threshold, we filter them out. Otherwise, we rectify their semantic categories by re-prediction. The generated pseudo labels thus become more reliable (+2.2\% mAP), as observed in the last two rows.
\end{itemize}

\begin{table}[]
\centering
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.0}
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccccc}
\specialrule{0.3pt}{0.1pt}{0pt}
                             
\hline
 Group & $\Tilde{S}^u$ & $\Tilde{O}^u$ & \textit{(C)} & \textit{(B)} & mAP & AP$_{50}$ & AP$_{25}$ \\
 \hline
  I & &  &  &  & 18.2 & 32.0 & 47.0\\
  II & \checkmark &  &  &  & 20.9 & 36.4	& 50.1\\
  III & & \checkmark &  &  & 19.7 & 35.2 &48.6 \\ 
  IV & \checkmark & \checkmark &  &  & 21.3 & 36.8 &50.2 \\ 
  V & \checkmark & \checkmark  & \checkmark  &  & 24.8 & 41.2 & 53.6\\
  VI & \checkmark& \checkmark & \checkmark & \checkmark & \textbf{27.0} & \textbf{44.1} & \textbf{56.2}\\
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Effects of different components of \ourMethod. $\Tilde{S}^u$ and $\Tilde{O}^u$ denote the pseudo semantic label and pseudo offset vector, respectively. \textit{(C)} denotes the proposal-based pseudo-label update and \textit{(B)} is the re-correction module (refer to modules \textbf{B} and \textbf{C} in Fig.~\ref{fig:overview}).}
\label{tab:abla_component}
\end{table}


\begin{table}[]
\centering
\renewcommand\tabcolsep{6.5pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{cccccc}
\specialrule{0.3pt}{0.1pt}{0pt}
                             
\hline
 \textit{sem-to-off} & \textit{off-to-sem} &  mAP & AP$_{50}$ & AP$_{25}$ & mIoU \\
 \hline
 \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\tiny \ding{52}}}$\square$ & \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\scriptsize \ding{56}}}$\square$ & 22.5 & 39.4 & 51.7 & 49.4 \\
  \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\scriptsize \ding{56}}}$\square$ & \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\tiny \ding{52}}}$\square$  &  21.7 & 38.7 & 50.5 & 52.0 \\
   \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\tiny \ding{52}}}$\square$ & \rlap{\raisebox{0.3ex}{\hspace{0.4ex}\tiny \ding{52}}}$\square$ & \textbf{27.0} & \textbf{44.1} & \textbf{56.2} & \textbf{54.9} \\
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Effects of mutual enhancement in \ourMethod{}. We disable the inter-label mutual enhancement by blocking either {\em semantic-to-offset} or {\em offset-to-semantic} enhancement during the self-training.} 
\label{tab:abla_interaction}
% \vspace{-0.1cm}
\end{table}

\begin{table}[]
\centering
\renewcommand\tabcolsep{4.5pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccc}
\specialrule{0.3pt}{0.1pt}{0pt}
\hline
 Group & \textit{Feature} & \textit{Augmentation} &  mAP & AP$_{50}$ & AP$_{25}$ \\
 \hline
  I & xyz+rgb & - & 22.3 & 38.0 & 51.8  \\
  II & xyz+b.feats. & - & 25.6 & 42.3 & 54.5\\

  III & xyz+b.feats. & trans. & 25.9 & 42.7 & 55.0 \\
  IV & xyz+b.feats. & mut. & 26.6 & 43.6 & 55.7\\
  V & xyz+b.feats. & trans.+mut. & \textbf{27.0} & \textbf{44.1} & \textbf{56.2} \\
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Comparisons with different input features and augmentation strategies of the re-correction module, where b.feats. denotes the backbone feature; trans. denotes the geometric transformation; and mut. denotes the geometric mutation.} 
\label{tab:abla_recorrection}
\vspace*{-0.4cm}
\end{table}

% Our \ourMethod~consists of the pseudo-label update and re-correction modules. To analyze the effects of the core modules, we experiment with different combinations and the results are shown in Table~ \ref{tab:abla_component}.
% We first set the baseline (Group I) as leveraging only the limited labels for supervision.
% In Group II and III, as discussed in Section 4.x, a naive strategy to generate the pseudo labels is by directly selecting the high-confidence pseudo-labels with a pre-defined threshold.
% Comparing I and III, a small gain (+1.5\%) is observed by introducing the pseudo instance center labels. 
% II observes a larger improvement(+2.7\%) compared to III, since \yxqnote{Explain the reason}. 
% Comparing IV with V, the obvious performance gain (+3.5\%) validates the effectiveness of our proposed semantic-instance interaction-based pseudo-label update module. 
% Thanks to the reciprocal promotion of both the pseudo semantic and instance center rather than simply leveraging the two pseudo labels, the performance of limited labeled data is evidently enhanced. 
% Since the pseudo-label generation inevitably contains unreliable labels that affects the network's learning procedure, we propose a learnable re-correction module to rectify the generated instance proposals. 
% The last two rows further validates the effect of re-correction module (+2.2\%). 

\vspace*{-2mm}
\noindent{\textbf{Effects of mutual enhancement.}}
\ourMethod~enables inter-label mutual enhancement by semantic-guided proposal generation and proposal-based pseudo-label update; see Sec.~\ref{subsec:method_c}. So, we disable two-way enhancement by altering either of the above modules and show ablation results in Table~\ref{tab:abla_interaction}.

To disable the offset-to-semantic enhancement, we simply produce the pseudo semantic labels by point-wise confidence thresholding, instead of adopting the proposal-based pseudo-label update. For a fair comparison, the generation strategy of the pseudo offset vector (Eqs.~\eqref{eq:pseudocenter} and~\eqref{eq:pseudooffset}) remains unchanged.
%To break the offset-to-semantic enhancement, we do not generate pseudo semantic labels during proposal-based pseudo-label update, rather producing them by point-wise confidence thresholding. The generation of pseudo offset vector remains the same (according to Eq.~\eqref{eq:pseudocenter} and Eq.~\eqref{eq:pseudooffset}).
% instead of from generate pseudo offset vectors based on instance proposals (Eq.~\eqref{eq:pseudocenter} and Eq.~\eqref{eq:pseudooffset}) but produce pseudo semantic labels by point-wise confidence thresholding. 
As observed in rows 1 and 3, it yields much inferior semantic predictions (-5.5\% mIoU) and thus a dramatic drop on instance segmentation accuracy (-4.5\% mAP). 

On the other hand, to block the semantic-to-offset enhancement, we change the clustering algorithm in the instance proposal generation procedure to a class-agnostic mechanism.
%To block the semantic-to-offset enhancement, we change the clustering algorithm to class-agnostic for instance proposal generation. 
As observed in Table~\ref{tab:abla_interaction} row 2 and row 3, despite the descent performance of semantic segmentation, its effect on guiding instance generation has been disabled, thus resulting in a 5.3\% mAP decrease in instance segmentation.
%Comparing row 2 with row 3, although the semantic mIoU is reasonably good, it cannot be utilized as prior to guide instance generation, thus resulting in a 5.3\% mAP decrease.
% although the semantic predictions can be benefited from proposal-level update (52\% mIoU at row 2), it cannot be utilized as prior to guide instance generation, thus the final accuracy dramatically decreases by 5.3\% mAP.




% During pseudo label updating, we explore the semantic-to-instance and the instance-to-semantic interaction, which correspond to the green and blue colored arrow in Fig.~\ref{fig:overview}. 
% To evaluate effect of each sub-module, we conduct experiments on ScanNet v2 validation set with 5\% labeled scenes. 

\vspace*{2mm}
\noindent{\textbf{Ablations for the re-correction module.}}
To further explore the impact of the re-correction module, we conduct experiments among the different settings shown in Table~\ref{tab:abla_recorrection}.
% To train the re-correction module, the input proposals can derive from the predicted proposals generated from the clustering operation. 
% In addition, the ground truth proposals can also be leveraged to increase the training samples, with a small gain from AP 25.6\% to 25.9\%. 

Regarding the input network features, we observe an obvious performance gain (+3.3\% mAP) with the features extracted from the backbone,~\ie, the output of Sparse U-Net of model $\Phi$, in comparison with the RGB features. It can be attributed to the captured contextual information in the network feature derived by the feature aggregation operation, which allows the re-correction module to leverage neighboring environments to boost the 3D object recognition.
%Regarding the input features of the network, we compare the features extracted from the backbone, \ie, the output of Sparse U-Net of model $\Phi$, with the RGB features, and observe an obvious performance gain (+3.3\% mAP). It can be attributed to the captured contextual information in backbone features by feature aggregation operation, which takes neighboring environments into consideration to make 3D object recognition easier.

Besides, we compare the effects of different data augmentation strategies. 
Comparing II and III, we find that simple geometric transformations such as rotation contribute a minor improvement.
Fortunately, by including and removing some adjacent points for geometric mutation, the instance proposals are enhanced with more variants. 
Group IV validates the effectiveness of our proposed geometric mutation strategy and Group V further enhances the performance %achieves the best performance 
by combining it with common augmentations.

Note that we only employ the re-correction module for proposal evaluation at the {\em pseudo-label update stage}; yet, it can also be used at test time to rectify the semantic class of the instance proposals onsite.  %before returning final results. 
In another comparison, we add the re-correction module to both the baseline (Sup-only in Table~\ref{tab:main_result}) and \ourMethod{} during the inference. It brings +2.5\% mAP over the baseline (still 6.3\% mAP lower than \ourMethod) but only +0.2\% mAP over \ourMethod. %We conjecture
This result manifests that \ourMethod~has been well optimized by the pseudo labels that are consistent with the re-correction module output. Thus, we do not need this module during the inference for computational efficiency.

\vspace*{2mm}
\noindent{\textbf{Ablations on different self-training rounds.}} \ourMethod{} typically converges in 3-4 rounds. The quality of the two sets of pseudo labels (Fig.~\ref{fig:pseudo_round} (a)) and the model performance (Table~\ref{tab:abla_round}) can both be gradually improved iteratively.

% \ourMethod~ gradually involves more and better pseudo labels for model training.
%can be iteratively promoted (Fig.~\ref{fig:pseudo_round}) and the model performance can also be improved accordingly (Table~\ref{tab:abla_round}).

    
\begin{table}[]
\centering
\renewcommand\tabcolsep{10.0pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\specialrule{0.3pt}{0.1pt}{0pt}
\hline
 \textit{Round} & 0 & 1 & 2 & 3 & 4 & 5 \\
 \hline
%   mAP & 18.2 & & & & & 27.0 \\
  1\% & 9.8 & 14.1 & 15.6 & 16.5 & 17.0 & 17.1 \\
  5\% & 32.0 & 38.7 & 42.3 & 43.7 & 44.1\ & 44.1 \\
  10\% & 42.8 & 45.8 & 48.3 & 49.5 & 49.7\ & 49.7 \\
  20\% & 47.9 & 51.2 & 52.0 & 52.8 & 52.9\ & 52.9 \\
  
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Performance at each self-training round on ScanNet v2, given \{1\%, 5\%, 10\%, 20\%\} ratios of labeled data. The round 0 denotes the ``sup-only'' baseline method. AP$_{50}$ = evaluation metric.} 
\label{tab:abla_round}
\vspace{-0.1cm}
\end{table}
    
    
    

\begin{table}[]
\centering
\renewcommand\tabcolsep{6.0pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ll|llll}
\specialrule{0.3pt}{0.1pt}{0pt}
\hline
& & \multicolumn{2}{c}{On Sem.} & \multicolumn{2}{c}{On Ins.} \\
\multirow{-2}{*}{Split} & \multirow{-2}{*}{Method} & mIoU   & mAcc & mAP & AP$_{50}$  \\
\hline
& CSC~\cite{hou2021exploring} & 29.3 & 40.0 & 7.1 & 13.0 \\
\multirow{-2}{*}{1\%} & \ourMethod{} & 31.0\cgaphl{+}{1.7}  & 41.2\cgaphl{+}{1.2} & \cellcolor{Gray}9.0\cgaphl{+}{1.9}  & \cellcolor{Gray}16.1\cgaphl{+}{3.1} \\
\hline
& CSC~\cite{hou2021exploring} & 49.1 & 57.2 & 20.9 & 36.7 \\
\multirow{-2}{*}{5\%} & \ourMethod{} & 54.9\cgaphl{+}{5.8} & 63.6\cgaphl{+}{6.4} & \cellcolor{Gray}24.0\cgaphl{+}{3.1} & \cellcolor{Gray}40.7\cgaphl{+}{4.0}\\
\hline
& CSC~\cite{hou2021exploring} & 59.5 & 69.3 & 27.3 & 45.0 \\
\multirow{-2}{*}{10\%} & \ourMethod{} & 61.1\cgaphl{+}{1.6} & 70.6\cgaphl{+}{1.3} & \cellcolor{Gray}29.2\cgaphl{+}{1.9} & \cellcolor{Gray}47.4\cgaphl{+}{2.4}\\
\hline
& CSC~\cite{hou2021exploring} & 64.1 & 73.1 & 30.6 & 50.3 \\
\multirow{-2}{*}{20\%} & \ourMethod{} & 66.5\cgaphl{+}{2.4} & 74.7\cgaphl{+}{1.6} & \cellcolor{Gray}31.8\cgaphl{+}{1.2} & \cellcolor{Gray}51.6\cgaphl{+}{1.3}\\
\specialrule{0.6pt}{0.1pt}{0pt}
\end{tabular}
}
\vspace{-0.2cm}
\caption{Performance improvement on both semantic segmentation and instance segmentation tasks compared with CSC. Gray regions denote that we degrade our semantic predictions results by using that from CSC, for a fair comparison on instance clustering quality.} 
\label{tab:compare_CSC}
\vspace{-0.4cm}
\end{table}

\subsection{Separate Semantic and Instance Improvement}
\ourMethod~can significantly benefit both the 3D semantic and instance segmentation in semi-supervised setting. In Table~\ref{tab:compare_CSC}, we further show the improvement on each task and compare it with the SOTA pre-training approach CSC~\cite{hou2021exploring}. In terms of semantic performance, our approach outperforms CSC in all data split settings (+1.6\%$ \sim $+5.8\% mIoU), thanks to the pseudo semantic labels.
In the view of the instance segmentation task, as our semantic branch has higher accuracy over CSC, for a fair comparison on the instance clustering quality, we discard our semantic results and directly replace it with the semantic predictions from CSC.
As presented in the gray regions, \ourMethod{}
still achieves better improvements with the help of pseudo offset supervisions for instance clustering.

% To elaborate the performance of our proposed approach compared to the SOTA CSC\cite{hou2021exploring} method in both semantic and instance segmentation tasks, we conduct the experiments on ScanNet v2 validation set given 1\%, 5\%, 10\% and 20\% limited annotation data.
% The comparison results is shown in Table~\ref{tab:compare_CSC}.
% In the view of semantic performance, due to the proposed pseudo-label updating and the re-correction module, our approach outperforms the CSC method in all the split settings (+1.6\%$ \sim $+5.8\%).
% In the view of instance segmentation task, since our semantic branch has higher accuracy over CSC, for fair comparison of instance clustering quality, we discard our semantic results and directly adopt the semantic predictions from CSC for replacement.
% As can be seen from the compared instance segmentation results, our method also achieves overwhelming improvements over CSC due to the semantic-to-instance update as well as the learnable re-correction module. 


